DeepRetrieval: Hacking Real Search Engines and Retrievers with Large Language Models via Reinforcement Learning

Information retrieval systems are crucial for enabling effective access to large document collections. Recent approaches have leveraged Large Language Models (LLMs) to enhance retrieval performance through query augmentation, but often rely on expensive supervised learning or distillation techniques that require significant computational resources and hand-labeled data. We introduce DeepRetrieval, a reinforcement learning (RL) approach that trains LLMs for query generation through trial and error without supervised data (reference query). Using retrieval metrics as rewards, our system generates queries that maximize retrieval performance. DeepRetrieval outperforms leading methods on literature search with 65.07% (vs. previous SOTA 24.68%) recall for publication search and 63.18% (vs. previous SOTA 32.11%) recall for trial search using real-world search engines. DeepRetrieval also dominates in evidence-seeking retrieval, classic information retrieval and SQL database search. With only 3B parameters, it outperforms industry-leading models like GPT-4o and Claude-3.5-Sonnet on 11/13 datasets. These results demonstrate that our RL approach offers a more efficient and effective paradigm for information retrieval. Our data and code are available at: https://github.com/pat-jj/DeepRetrieval.

==> contribution_statement.tex <==
\textbf{P. Jiang} developed the DeepRetrieval framework and conducted the preliminary study on literature search using a search engine. He was responsible for writing the abstract, introduction, methodology, main results, and discussion sections. He carried out all experiments on literature search, evidence-seeking retrieval, and sparse retrieval across the MS-H, MS-S, and MS-T datasets. Additionally, he conducted the knowledge injection and think/query length studies and created all figures presented in the paper.

\textbf{J. Lin} provided guidance on the VERL framework (the base architecture for applying the RL approach) and conducted the majority of the sparse and dense retrieval experiments (84 out of 96) following P. Jiang's preliminary findings on search engine retrieval. He drafted the complete methodology section and wrote the analysis on sparse and dense retrieval in the main results and discussion sections.

\textbf{L. Cao} implemented the SQL database search component and conducted all experiments on the BIRD and Spider datasets. He also constructed the MS-H, MS-S, and MS-T subsets and performed dense retrieval experiments on these datasets. Additionally, he contributed to the main results and discussion sections related to SQL retrieval.

\textbf{R. Tian} participated in project discussions, conducted the literature review, and authored most content of the Related Work section.

\textbf{S. Kang} joined the project after the preliminary results on search engine retrieval and proposed datasets for evaluating the method's performance. He also suggested relevant papers for discussion in the Related Work section.

\textbf{Z. Wang} initiated the idea of applying LLM+RL to the literature search task and contributed to project discussions. He also proposed the performance visualization format and assisted in paper editing.

\textbf{Prof. J. Sun} and \textbf{Prof. J. Han}, provided guidance on framework design, offered suggestions on paper writing, and contributed to paper editing.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old/old_methodology_section.tex <==
\section{DeepRetrieval}

DeepRetrieval is a 

builds upon recent advances in reinforcement learning for LLMs, applying this paradigm to the specific task of query augmentation for information retrieval. Our methodology is directly inspired by DeepSeek-R1-Zero \citep{deepseekai2025deepseekr1incentivizingreasoningcapability}, which demonstrated that RL can be used to train models with advanced reasoning capabilities without relying on supervised data. Figure \ref{fig:approach} illustrates an abstractive overall architecture of our system.

\subsection{Problem Formulation}
Let $D$ be a collection of documents and $q$ be a user query. The goal of an information retrieval system is to return a set of documents $D_q \subset D$ that are relevant to $q$. In query augmentation, the original query $q$ is transformed into an augmented query $q'$ that is more effective at retrieving relevant documents.

Traditionally, this augmentation process is learned through supervised learning, where pairs of $(q, q')$ are provided as training data. In contrast, our approach uses reinforcement learning, where the model learns to generate effective augmented queries through trial and error, similar to how DeepSeek-R1-Zero learns to solve reasoning problems.

\subsection{Reinforcement Learning Framework}
We formulate the query augmentation task as a reinforcement learning problem:

\begin{itemize}
    \item \textbf{State}: The user's original query $q$
    \item \textbf{Action}: The augmented query $q'$ generated by the model
    \item \textbf{Reward}: The recall achieved when using $q'$ to retrieve documents
\end{itemize}

The model is trained to maximize the expected reward, i.e., to generate augmented queries that achieve high recall. This direct optimization for the end goal differs from supervised approaches, which optimize for similarity to human-generated or larger-model-generated augmentations.

\subsection{Model Architecture and Output Structure}
We utilize Qwen-2.5-3B-Instruct~\citep{yang2024qwen2} as the base LLM for our system. The model takes the user query as input and generates an augmented query. The model is structured to first generate reasoning steps in a \texttt{<think>} section, followed by the final augmented query in an \texttt{<answer>} section in JSON format. This structured generation allows the model to consider various aspects of the query and explore different augmentation strategies before finalizing its response.

For our initial experiments, we focused on medical literature retrieval using a specialized prompt based on the PICO framework (see Appendix \ref{appendix:prompt} for details). The JSON format with Boolean operators (AND, OR) and appropriate parentheses for grouping is required for compatibility with search systems. However, our methodology is general and can be applied to traditional IR datasets with appropriate modifications to the prompt and query format.

\subsection{Reward Mechanism}
Our reward function is designed to directly optimize for retrieval performance. The process works as follows:

\begin{enumerate}
    \item The model generates an augmented query in response to a PICO framework query
    \item The augmented query is executed against a document collection (PubMed or ClinicalTrials.gov)
    \item Recall is computed as the proportion of relevant documents retrieved
    \item A composite reward is calculated based on:
        \begin{itemize}
            \item Format correctness (JSON structure, proper tagging)
            \item Retrieval recall, with higher rewards for better recall
        \end{itemize}
\end{enumerate}

Specifically, our reward function uses a tiered scoring system for recall performance, as shown in Table \ref{tab:reward}.

\begin{table}[h]
\centering
\begin{tabular}{lccccccc}
\toprule
Recall
&$\geq 0.7$ & $\geq 0.5$ & $\geq 0.4$ & $\geq 0.3$ & $\geq 0.1$ & $\geq 0.05$ & $< 0.05$ \\
\midrule
Reward & +5.0 & +4.0 & +3.0 & +1.0 & +0.5 & +0.1 & -3.5 \\
\bottomrule
\end{tabular}
\caption{Reward tiers based on recall performance. Higher recall values receive significantly larger rewards, incentivizing the model to generate more effective queries.}
\label{tab:reward}
\end{table}

Additionally, correct formatting receives +1 point, while incorrect formatting receives -4 points. Importantly, if the format is incorrect (missing tags, improper JSON structure, etc.), the answer reward is not computed at all, resulting in only the formatting penalty. This reward structure strongly encourages the model to generate well-formed queries that maximize recall while adhering to the required output format.


\subsection{Training Process}
Our training process follows these steps:

\begin{enumerate}
    \item Initialize the model with pre-trained weights
    \item For each query in the training set:
        \begin{enumerate}
            \item Generate an augmented query
            \item Execute the query against the search system
            \item Compute the recall (proportion of relevant documents retrieved)
            \item Use the recall-based reward to update the model
        \end{enumerate}
    \item Repeat until convergence
\end{enumerate}

This process allows the model to learn effective query augmentation strategies directly from the retrieval performance, without requiring explicit supervision. The model gradually improves its ability to transform PICO framework queries into effective search terms that maximize recall of relevant medical literature.

==> tables/task_0_perf.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
&& \multicolumn{2}{c}{\textbf{Literature Mining}} & \multicolumn{9}{c}{\textbf{Evidence-Seeking Retrieval}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-13} 
& &\textbf{Publication} &\textbf{CinicalTrials} &\multicolumn{3}{c}{\textbf{NQ}} &\multicolumn{3}{c}{\textbf{TriviaQA}} &\multicolumn{3}{c}{\textbf{SQuAD}}\\ 
& ``Think'' & Recall & Recall  &H@1 &H@5 &H@20 &H@1 &H@5 &H@20 &H@1 &H@5 &H@20 \\
\midrule
\textbf{Original Query} &-    &10.36  &18.01 & 21.86 &43.77 &62.99 &48.23 &66.29 &76.41 &36.93 &57.61 &71.31\\
\midrule
\multicolumn{4}{l}{\textbf{Proprietary Models}}
\\[2pt]
\hdashline[2pt/2pt] \\ [-9pt]
\multirow{2}{*}{GPT-3.5} & \xmark & 4.01 & 3.37 &25.20 &47.53 &66.28 &47.46 &66.77 &76.73 &33.86 &54.85 &69.47 \\
 & \cmark & 18.68 & 13.94 &24.26 &45.98 &63.93 &45.80 &64.30 &74.19 &30.32 &50.35 &64.36  \\
 \multirow{2}{*}{GPT-4o} & \xmark & 5.79 & 6.74 &29.14 &56.16 &69.33 &53.36 &70.07 &78.72 &32.95 &52.18 &66.72 \\
 & \cmark & 19.72 & 14.26 &35.78 &57.50 &72.21 &59.63 &73.31 &80.53 &30.38 &49.85 &64.43 \\[2pt]
\hdashline[2pt/2pt] \\ [-9pt]
\multirow{2}{*}{Claude-3-Haiku} & \xmark & 10.98 & 11.59 &24.95 &48.14 &65.54 &49.04 &67.65 &77.33 &33.19 &54.31 &68.78 \\
 & \cmark  & 20.92 & 24.68 &26.17 &48.55 &66.37 &48.81 &67.90 &77.67 &33.33 &54.08 &68.44 \\
\multirow{2}{*}{Claude-3.5-Sonnet} & \xmark && &37.22 &56.92 &72.77 &60.84 &73.80 &80.57 &30.25 &49.82 &64.71  \\
 & \cmark && &35.73 &57.06 &72.52 &57.14 &71.70 &79.74 & \\
\midrule
\multicolumn{4}{l}{\textbf{Open-source Models}} \\
Mistral-7B & \xmark & 7.18 & 8.08 \\
LEADS & \cmark & 24.68 & 32.11 &- &- &- &- &- &- &- &- &-\\

\multirow{2}{*}{Qwen2.5-3B-Inst}  & \xmark  \\

& \cmark &6.59 &6.09 &25.04 &45.78 &63.40 &47.51 &65.58 &75.81 &28.42 &46.42 &61.30 \\
\midrule
\textbf{Ours} \\
DeepRetrieval (3B) & \cmark & \textbf{60.88} & \textbf{63.18} &\textbf{32.46} &\textbf{56.12} &\textbf{71.87} \\
\bottomrule
\end{tabular}}
\caption{\textbf{Performance on literature mining and evidence-seeking retrieval.} We evaluate performance across multiple datasets. For Publication and CinicalTrials, we use Recall@3K as the metric~\citep{wang2025foundationmodelhumanaicollaboration}, with the PubMed and ClinicalTrials.gov search engines serving as retrievers, respectively. For evidence-seeking retrieval (Natural Questions (NQ), TriviaQA, and SQuAD), we assess performance by measuring ``retrieval accuracy'' (answer span hits) \citep{lin2021pyserini,ma2021replication}, using BM25 as the base retriever.}
\label{tab:results}

\end{table}

==> tables/task_0_perf_1.tex <==
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccccccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Literature Searching}} & \multicolumn{9}{c}{\textbf{Evidence-Seeking Retrieval}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-12} 
&\textbf{Publication} &\textbf{CinicalTrials} &\multicolumn{3}{c}{\textbf{NQ}} &\multicolumn{3}{c}{\textbf{TriviaQA}} &\multicolumn{3}{c}{\textbf{SQuAD}}\\  & Recall & Recall  &H@1 &H@5 &H@20 &H@1 &H@5 &H@20 &H@1 &H@5 &H@20 \\
\midrule
Original Query  &10.36  &18.01 & 21.9 &43.8 &63.0 &48.2 &66.3 &76.4 &36.5 &57.4 &71.1\\
\midrule
% \multicolumn{12}{c}{\textbf{Proprietary Models}}
% \\[2pt]
% \hdashline[2pt/2pt] \\ [-9pt]
GPT-3.5   & 18.68 & 13.94 &24.3 &46.0 &63.9 &45.8 &64.3 &74.2 &31.6 &52.4 &66.6  \\
\quad w/o reasoning & 4.01 & 3.37 &25.2 &47.5 &66.3 &47.5 &66.8 &76.7 &33.9 &54.9 &69.5 \\
\quad w/o answer inject &- &- &22.2 &44.0 &62.3 &37.5 &55.9 &66.9 &29.3 &49.5 &63.9
\\[2pt]
\hdashline[2pt/2pt] \\ [-9pt]
GPT-4o  & 19.72 & 14.26 &35.8 &57.5 &72.2 &59.6 &73.3 &80.5 &30.4 &49.9 &64.4 \\
 \quad w/o reasoning  & 5.79 & 6.74 &29.1 &56.2 &69.3 &53.4 &70.1 &78.7 &33.0 &52.2 &66.7 \\
 \quad w/o answer inject  & - &- &27.4 &51.8 &68.4 &42.1 &61.2 &71.5 &25.5 &45.9 &61.8\\[2pt]
\hdashline[2pt/2pt] \\ [-9pt]
Claude-3-Haiku    & 20.92 & 24.68 &26.2 &48.6 &66.4 &48.8 &67.9 &77.7 &33.3 &54.1 &68.4 \\
 \quad w/o reasoning & 10.98 & 11.59 &25.0 &48.1 &65.5 &49.0 &67.7 &77.3 &33.2 &54.3 &68.8 \\
  \quad w/o answer inject &- &- &22.7 &45.6 &63.1 &38.1 &57.0 &68.1 &30.7 &51.3 &65.8\\
 [2pt]
\hdashline[2pt/2pt] \\ [-9pt]
Claude-3.5-Sonnet  &21.06 &24.88 &35.7 &57.1 &72.5 &57.1 &71.7 &79.7 &28.5 &48.1 &63.5 \\
  \quad w/o reasoning &12.56 &13.77 &37.2 &56.9 &72.8 &60.8 &73.8 &80.6 &30.3 &49.8 &64.7  \\
 \quad w/o answer inject  &-&- &27.6 &52.0 &69.7 &42.8 &61.9 &72.6 &24.1 &44.6 &61.2 \\
\midrule
% \multicolumn{4}{l}{\textbf{Open-source Models}} \\
Mistral$_{\text{7B}}$  & 7.18 & 8.08 \\
LEADS  & \underline{24.68} & \underline{32.11} &- &- &- &- &- &- &- &- &-\\
 [2pt]
\hdashline[2pt/2pt] \\ [-9pt]
Qwen2.5$_{\text{3B-Inst}}$   
 &6.59 &6.09 &25.0 &45.8 &63.4 &44.4 &61.2 &70.9 &28.4 &46.4 &61.3 \\
 \quad w/o reasoning \\
 \quad w/o answer inject  &-&- \\
\midrule
% \textbf{Ours} \\
DeepRetrieval$_{\text{3B}}$  & \textcolor{red}{\textbf{60.88}} & \textcolor{red}{\textbf{63.18}} &\textbf{35.5} &\textbf{57.5} &\textbf{72.7} &58.4 &73.2 &80.5 &38.5 &59.4 &72.9 \\
\quad w/o reasoning & 51.90 &53.31 \\
\quad w/o answer inject  &-&- \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\item{- \textbf{[w/o reasoning]}} Removes the thinking process ($<$think$>$...$<$/think$>$), forcing the model to generate queries directly.
    
\item{- \textbf{[w/o answer inject]}} This setting addresses an issue in evidence-seeking retrieval where LLMs input answer information to the generated queries based on prior knowledge. We implement a postprocessing where an auxiliary LLM analyzes the generated query, identifies answer injections, and removes the answer terms to ensure a more fair evaluation. See more details in Appendix \ref{ap:injection}.


\end{tablenotes}
\end{threeparttable}
}
\caption{\textbf{Performance on literature searching and evidence-seeking retrieval.} We evaluate performance across multiple datasets. For Publication and CinicalTrials, we use Recall@3K as the metric~\citep{wang2025foundationmodelhumanaicollaboration}, with the PubMed and ClinicalTrials.gov search engines serving as retrievers, respectively. For evidence-seeking retrieval (Natural Questions (NQ), TriviaQA, and SQuAD), we assess performance by measuring ``retrieval accuracy'' H@N (answer span hits) \citep{lin2021pyserini,ma2021replication}, using BM25 as the base retriever.}
\label{tab:results}

\end{table}
